Pruning Laws for Large Language Models

Scaling up model parameters and training data consistently improves the performance of large language models (LLMs), but at the cost of rapidly growing memory and compute requirements, which makes deployment on resource-limited hardware infeasible. Model pruning, a widely used compression technique, reduces inference costs by removing redundant parameters. However, its impact on downstream performance remains unpredictable and is typically assessed only through costly empirical sweeps. To address this gap, we introduce pruning laws, simple and interpretable scaling relations that connect a pruned LLM's post-pruning performance to its unpruned performance and pruning ratio. Across ten LLMs (1.3B-30B parameters), a 20B mixture-of-experts model, three pruning strategies (unstructured, width, and depth), and eight diverse tasks, we show that pruning laws achieve strong predictive accuracy (average extrapolation error less than 7%), reliably quantify performance degradation, and identify critical pruning thresholds beyond which recovery is infeasible. Moreover, we demonstrate that the functional form transfers across dense and mixture-of-experts architectures, pruning methods, and unseen models in zero-shot and one-shot setups, with task- and method-specific coefficients that vary in interpretable ways. These results provide both researchers and practitioners with a principled framework to select pruning strategies, estimate safe pruning ratios without exhaustive tuning, and deploy LLMs efficiently under real-world compute and latency constraints.

==> tables/all_runtime.tex <==
% Table generated by Excel2LaTeX from sheet 'all_runtime'
\begin{table}[htbp]
  \centering
  \scalebox{0.8}{
    \begin{tabular}{crrrr}
    \toprule
    \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{l}{\textbf{Pruning Ratio}} & \multicolumn{1}{l}{\textbf{DepthPruning}} & \multicolumn{1}{l}{\textbf{Unstructured}} & \multicolumn{1}{l}{\textbf{WidthPruning}} \\
    \midrule
    \multirow{9}[0]{*}{LLaMA-13B} & 0.1   & 1.42  & 1.15  & 0.98 \\
          & 0.2   & 1.52  & 1.15  & 1.04 \\
          & 0.3   & 1.60  & 1.15  & 1.15 \\
          & 0.4   & 1.72  & 1.16  & 1.19 \\
          & 0.5   & 1.84  & 1.16  & 1.15 \\
          & 0.6   & 1.84  & 1.17  & 1.28 \\
          & 0.7   & 1.84  & 1.18  & 1.36 \\
          & 0.8   & 1.84  & 1.18  & 1.44 \\
          & 0.9   & 1.84  & 1.19  & 1.36 \\
    \cdashline{1-5}
    \multirow{9}[0]{*}{LLaMA-7B} & 0.1   & 1.34  & 1.24  & 1.00 \\
          & 0.2   & 0.85  & 1.24  & 0.94 \\
          & 0.3   & 1.28  & 1.24  & 1.00 \\
          & 0.4   & 1.63  & 1.24  & 0.94 \\
          & 0.5   & 1.63  & 1.25  & 1.02 \\
          & 0.6   & 1.63  & 1.25  & 1.05 \\
          & 0.7   & 1.63  & 1.25  & 1.01 \\
          & 0.8   & 1.63  & 1.25  & 1.05 \\
          & 0.9   & 1.63  & 1.26  & 0.98 \\
    \cdashline{1-5}
    \multirow{9}[0]{*}{OPT-13B} & 0.1   & 1.07  & 1.22  & 0.90 \\
          & 0.2   & 1.20  & 1.22  & 0.98 \\
          & 0.3   & 1.35  & 1.22  & 0.98 \\
          & 0.4   & 1.54  & 1.23  & 1.11 \\
          & 0.5   & 1.80  & 1.24  & 1.10 \\
          & 0.6   & 2.13  & 1.24  & 1.17 \\
          & 0.7   & 2.74  & 1.24  & 1.26 \\
          & 0.8   & 3.51  & 1.25  & 1.37 \\
          & 0.9   & 5.05  & 1.26  & 1.18 \\
    \cdashline{1-5}
    \multirow{9}[0]{*}{OPT-2.7B} & 0.1   & 1.40  & 1.29  & 0.90 \\
          & 0.2   & 1.30  & 1.30  & 0.82 \\
          & 0.3   & 1.29  & 1.29  & 0.86 \\
          & 0.4   & 1.43  & 1.29  & 0.88 \\
          & 0.5   & 1.75  & 1.29  & 0.91 \\
          & 0.6   & 1.75  & 1.30  & 0.84 \\
          & 0.7   & 1.75  & 1.31  & 0.90 \\
          & 0.8   & 1.75  & 1.30  & 0.87 \\
          & 0.9   & 1.75  & 1.31  & 0.86 \\
    \cdashline{1-5}
    \multirow{9}[0]{*}{OPT-6.7B} & 0.1   & 1.07  & 1.19  & 0.94 \\
          & 0.2   & 1.17  & 1.20  & 0.88 \\
          & 0.3   & 1.32  & 1.19  & 0.93 \\
          & 0.4   & 1.49  & 1.20  & 0.98 \\
          & 0.5   & 1.79  & 1.20  & 1.02 \\
          & 0.6   & 2.13  & 1.20  & 1.01 \\
          & 0.7   & 2.63  & 1.21  & 1.08 \\
          & 0.8   & 3.44  & 1.21  & 1.08 \\
          & 0.9   & 5.01  & 1.22  & 1.04 \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Inference speedup over unpruned LLMs for different pruning ratios.}
  \label{tab:all_runtime}%
\end{table}%


==> tables/glossary.tex <==
\begin{table}[htbp]
  \centering
  \caption{Glossary of all appendix tables and figures.}
  \scalebox{0.9}{
    \begin{tabular}{llp{20em}}
    \toprule
    \bf Description & \bf Granularity & \bf Reference \\
    \midrule
    Base LLM performance results & Model and Task &  Table~\ref{tab:base_model_results} \\
    \midrule

    \multirow{6}{*}{Empirical results of pruned LLMs} & Model and Task & Table~\ref{tab:compressed_model_results} (mean performance across pruning methods)\\
                                                        & Model and Task & Figure~\ref{fig:all_performance} (performance with all methods)\\
                                                        & Model and Task & Figure~\ref{fig:unstrct_performance} (performance with unstructured pruning)\\
                                                        & Model and Task & Figure~\ref{fig:depth_performance} (performance with depth pruning)\\
                                                        & Model and Task & Figure~\ref{fig:width_performance} (performance with width pruning)\\
                                                        & Model and Task & Figure~\ref{fig:calibfree_performance} (performance with calibration-free width pruning)\\

    \midrule
    \multirow{3}{*}{Pruning laws of performance} & Model and Task & Table~\ref{tab:model_level_scaling_laws_full} \\
                                                & Method and Task & Table~\ref{tab:method_level_scaling_laws_full}\\
                                                & Model, Method and Task & Table~\ref{tab:method_model_level_scaling_laws_full} and Table~\ref{tab:method_model_level_scaling_laws_full_robust}\\
    \midrule 
    
    Pruning law of runtime efficiency & Model and Method & Table~\ref{tab:methodwise_runtime_scaling_laws} \\
    \midrule

    \multirow{5}{*}{Fitted pruning law of performance} & Model and Task & Figure~\ref{fig:taskwise_scaling_fit}\\
                                                                & Model and Task & Figure~\ref{fig:unstrct_taskwise_scaling_fit} (unstructured pruning)\\
                                                                & Model and Task & Figure ~\ref{fig:depth_taskwise_scaling_fit} (depth pruning)\\
                                                                & Model and Task & Figure ~\ref{fig:width_taskwise_scaling_fit} (width pruning)\\
                                                                & Model and Task & Figure ~\ref{fig:calibfree_taskwise_scaling_fit} (calibration-free width pruning)\\
    \midrule

    \multirow{3}{*}{Fitted pruning law of runtime} & Model & Figure~\ref{fig:runtime_unstrct} (unstructured pruning) \\
                                                                & Model & Figure ~\ref{fig:runtime_depth} (depth pruning)\\
                                                                & Model & Figure ~\ref{fig:runtime_width} (width pruning)\\
    \midrule
    
    Critical pruning ratio & Model, Method and Task & Figure~\ref{fig:criticalratio_methodwise} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:glossary}%
\end{table}%


==> tables/method_model_task_level.tex <==
\begin{table}[htbp]
  \centering
  \scalebox{0.8}{
    \begin{tabular}{lccllrrr}
    \toprule
    \textbf{Task} & \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{l}{\textbf{Method}} & \textbf{$\alpha$} & \textbf{$P_0$} & \multicolumn{1}{l}{\textbf{Adj $R^2$}} & \multicolumn{1}{l}{\textbf{F Statistic}} & \multicolumn{1}{l}{\textbf{Test Error}} \\
    \midrule
    QA    & \multirow{4}[0]{*}{OPT-2.7B} & \multirow{20}[0]{*}{Unstructured} & 2.63 $\pm$ 0.42 & 3.08 $\pm$ 0.46 & 0.83  & 39.87 & 0.15 \\
    Reasoning &       &       & 0.23 $\pm$ 0.02 & 1.15 $\pm$ 0.03 & 0.92  & 95.53 & 0.07 \\
    Language &       &       & 0.8 $\pm$ 0.07 & 1.32 $\pm$ 0.08 & 0.93  & 114.16 & 0.13 \\
    Average &       &       & 0.39 $\pm$ 0.03 & 1.17 $\pm$ 0.04 & 0.95  & 139.41 & 0.09 \\
    QA    & \multirow{4}[0]{*}{OPT-6.7B} &       & 2.77 $\pm$ 0.53 & 3.82 $\pm$ 0.62 & 0.79  & 27.24 & 0.23 \\
    Reasoning &       &       & 0.27 $\pm$ 0.03 & 1.17 $\pm$ 0.03 & 0.94  & 103.33 & 0.08 \\
    Language &       &       & 0.87 $\pm$ 0.12 & 1.44 $\pm$ 0.14 & 0.88  & 51.50 & 0.19 \\
    Average &       &       & 0.44 $\pm$ 0.05 & 1.22 $\pm$ 0.06 & 0.91  & 76.15 & 0.13 \\
    QA    & \multirow{4}[0]{*}{LLaMA-7B} &       & 2.71 $\pm$ 0.49 & 3.65 $\pm$ 0.55 & 0.78  & 30.05 & 0.31 \\
    Reasoning &       &       & 0.37 $\pm$ 0.05 & 1.18 $\pm$ 0.05 & 0.88  & 59.14 & 0.14 \\
    Language &       &       & 0.95 $\pm$ 0.08 & 1.34 $\pm$ 0.09 & 0.95  & 139.71 & 0.16 \\
    Average &       &       & 0.53 $\pm$ 0.06 & 1.22 $\pm$ 0.07 & 0.91  & 77.53 & 0.17 \\
    QA    & \multirow{4}[0]{*}{OPT-13B} &       & 2.65 $\pm$ 0.51 & 3.5 $\pm$ 0.56 & 0.77  & 27.53 & 0.24 \\
    Reasoning &       &       & 0.28 $\pm$ 0.03 & 1.18 $\pm$ 0.03 & 0.93  & 114.94 & 0.10 \\
    Language &       &       & 0.94 $\pm$ 0.13 & 1.47 $\pm$ 0.14 & 0.86  & 52.26 & 0.19 \\
    Average &       &       & 0.45 $\pm$ 0.05 & 1.23 $\pm$ 0.05 & 0.92  & 94.66 & 0.14 \\
    QA    & \multirow{4}[0]{*}{LLaMA-13B} &       & 2.77 $\pm$ 0.53 & 3.87 $\pm$ 0.58 & 0.77  & 27.73 & 0.36 \\
    Reasoning &       &       & 0.38 $\pm$ 0.05 & 1.19 $\pm$ 0.05 & 0.89  & 66.52 & 0.15 \\
    Language &       &       & 0.98 $\pm$ 0.1 & 1.4 $\pm$ 0.11 & 0.93  & 102.91 & 0.20 \\
    Average &       &       & 0.55 $\pm$ 0.06 & 1.25 $\pm$ 0.07 & 0.90  & 73.61 & 0.19 \\
    \cdashline{1-8}
    QA    & \multirow{4}[0]{*}{OPT-2.7B} & \multirow{19}[0]{*}{DepthPruning} & 1.51 $\pm$ 0.62 & 0.02 $\pm$ 0.69 & 0.38  & 5.85  & 0.06 \\
    Reasoning &       &       & 0.06 $\pm$ 0.02 & 0.79 $\pm$ 0.02 & 0.43  & 7.03  & 0.06 \\
    Language &       &       & 0.19 $\pm$ 0.07 & 0.27 $\pm$ 0.08 & 0.46  & 7.95  & 0.08 \\
    Average &       &       & 0.07 $\pm$ 0.03 & 0.57 $\pm$ 0.03 & 0.45  & 7.42  & 0.07 \\
    QA    & \multirow{4}[0]{*}{OPT-6.7B} &       & 1.8 $\pm$ 1.01 & 0.03 $\pm$ 1.12 & 0.21  & 3.18  & 0.00 \\
    Reasoning &       &       & 0.14 $\pm$ 0.07 & 0.78 $\pm$ 0.08 & 0.24  & 3.51  & 0.18 \\
    Language &       &       & 0.58 $\pm$ 0.23 & 0.35 $\pm$ 0.26 & 0.40  & 6.33  & 0.06 \\
    Average &       &       & 0.22 $\pm$ 0.12 & 0.61 $\pm$ 0.13 & 0.24  & 3.58  & 0.15 \\
    QA    & \multirow{3}[0]{*}{LLaMA-7B} &       & 1.2 $\pm$ 0.5 & 0.33 $\pm$ 0.55 & 0.37  & 5.78  & 0.18 \\
    Reasoning &       &       & 0.13 $\pm$ 0.06 & 0.78 $\pm$ 0.06 & 0.35  & 5.40  & 0.15 \\
    Language &       &       & 0.23 $\pm$ 0.11 & 0.31 $\pm$ 0.12 & 0.31  & 4.61  & 0.16 \\
    Average &       &       & 0.2 $\pm$ 0.09 & 0.62 $\pm$ 0.09 & 0.35  & 5.32  & 0.17 \\
    Reasoning &       &       & 0.01 $\pm$ 0.01 & 0.63 $\pm$ 0.01 & 0.15  & 2.37  & 0.04 \\
    Language &       &       & 0.1 $\pm$ 0.06 & 0.15 $\pm$ 0.06 & 0.23  & 3.35  & 0.02 \\
    Average &       &       & 0.02 $\pm$ 0.01 & 0.43 $\pm$ 0.01 & 0.22  & 3.22  & 0.03 \\
    QA    & \multirow{4}[0]{*}{LLaMA-13B} &       & 2.59 $\pm$ 0.8 & 0.11 $\pm$ 0.89 & 0.54  & 10.45 & 0.01 \\
    Reasoning &       &       & 0.15 $\pm$ 0.06 & 0.73 $\pm$ 0.07 & 0.37  & 5.72  & 0.15 \\
    Language &       &       & 0.29 $\pm$ 0.12 & 0.25 $\pm$ 0.13 & 0.40  & 6.37  & 0.07 \\
    Average &       &       & 0.14 $\pm$ 0.05 & 0.49 $\pm$ 0.06 & 0.44  & 7.37  & 0.10 \\
    \cdashline{1-8}
    QA    & \multirow{4}[0]{*}{OPT-2.7B} & \multirow{20}[0]{*}{WidthPruning} & 3.0 $\pm$ 0.53 & 0.42 $\pm$ 0.59 & 0.80  & 32.30 & 0.01 \\
    Reasoning &       &       & 0.2 $\pm$ 0.05 & 0.95 $\pm$ 0.06 & 0.64  & 15.03 & 0.11 \\
    Language &       &       & 0.76 $\pm$ 0.1 & 0.71 $\pm$ 0.11 & 0.87  & 56.24 & 0.04 \\
    Average &       &       & 0.32 $\pm$ 0.08 & 0.81 $\pm$ 0.09 & 0.67  & 17.56 & 0.10 \\
    QA    & \multirow{4}[0]{*}{OPT-6.7B} &       & 3.37 $\pm$ 0.56 & 0.85 $\pm$ 0.62 & 0.82  & 36.58 & 0.03 \\
    Reasoning &       &       & 0.26 $\pm$ 0.05 & 0.99 $\pm$ 0.06 & 0.77  & 27.21 & 0.08 \\
    Language &       &       & 0.83 $\pm$ 0.08 & 0.8 $\pm$ 0.08 & 0.94  & 118.73 & 0.03 \\
    Average &       &       & 0.4 $\pm$ 0.07 & 0.88 $\pm$ 0.08 & 0.78  & 30.19 & 0.09 \\
    QA    & \multirow{4}[0]{*}{LLaMA-7B} &       & 3.33 $\pm$ 0.37 & 1.1 $\pm$ 0.41 & 0.91  & 79.60 & 0.03 \\
    Reasoning &       &       & 0.25 $\pm$ 0.07 & 0.84 $\pm$ 0.07 & 0.63  & 14.34 & 0.14 \\
    Language &       &       & 0.82 $\pm$ 0.09 & 0.59 $\pm$ 0.1 & 0.91  & 80.98 & 0.04 \\
    Average &       &       & 0.38 $\pm$ 0.09 & 0.73 $\pm$ 0.1 & 0.70  & 19.61 & 0.11 \\
    QA    & \multirow{4}[0]{*}{OPT-13B} &       & 3.48 $\pm$ 0.39 & 1.91 $\pm$ 0.43 & 0.91  & 81.04 & 0.06 \\
    Reasoning &       &       & 0.28 $\pm$ 0.04 & 1.04 $\pm$ 0.05 & 0.85  & 45.94 & 0.07 \\
    Language &       &       & 0.84 $\pm$ 0.07 & 0.87 $\pm$ 0.08 & 0.95  & 151.76 & 0.03 \\
    Average &       &       & 0.43 $\pm$ 0.06 & 0.97 $\pm$ 0.07 & 0.85  & 48.01 & 0.07 \\
    QA    & \multirow{4}[0]{*}{LLaMA-13B} &       & 3.06 $\pm$ 0.46 & 1.22 $\pm$ 0.51 & 0.84  & 43.97 & 0.04 \\
    Reasoning &       &       & 0.29 $\pm$ 0.07 & 0.87 $\pm$ 0.08 & 0.65  & 16.09 & 0.15 \\
    Language &       &       & 0.83 $\pm$ 0.1 & 0.59 $\pm$ 0.11 & 0.89  & 66.53 & 0.05 \\
    Average &       &       & 0.43 $\pm$ 0.09 & 0.77 $\pm$ 0.1 & 0.72  & 21.24 & 0.11 \\
    \bottomrule
    \end{tabular}%
    }
  \caption{Coefficients of method-model-task level pruning laws.}
  \label{tab:method_model_level_full}%
\end{table}%


==> tables/method_task_level.tex <==
% Table generated by Excel2LaTeX from sheet 'method_task_level_fitting_laws'
\begin{table}[htbp]
  \centering
  \scalebox{1}{
    \begin{tabular}{llllrrr}
    \toprule
    \textbf{Task} & \textbf{Method} & \textbf{$\alpha$} & \textbf{$P_0$} & \multicolumn{1}{l}{\textbf{Adj $R^2$}} & \multicolumn{1}{l}{\textbf{F Statistic}} & \multicolumn{1}{l}{\textbf{Test Error}} \\
    \midrule
    \textbf{QA} & Unstructured & 2.71 $\pm$ 0.2 & 3.56 $\pm$ 0.22 & 0.81  & 183.76 & 0.25 \\
    \textbf{Reasoning} & Unstructured & 0.31 $\pm$ 0.02 & 1.17 $\pm$ 0.02 & 0.85  & 252.22 & 0.12 \\
    \textbf{Language} & Unstructured & 0.91 $\pm$ 0.04 & 1.39 $\pm$ 0.05 & 0.91  & 418.66 & 0.18 \\
    \textbf{Average} & Unstructured & 0.47 $\pm$ 0.03 & 1.22 $\pm$ 0.03 & 0.90  & 370.20 & 0.15 \\
    \cdashline{1-7}
    \textbf{QA} & DepthPruning & 1.42 $\pm$ 0.43 & 0.03 $\pm$ 0.48 & 0.18  & 10.70 & 0.02 \\
    \textbf{Reasoning} & DepthPruning & 0.1 $\pm$ 0.03 & 0.74 $\pm$ 0.03 & 0.22  & 13.11 & 0.09 \\
    \textbf{Language} & DepthPruning & 0.28 $\pm$ 0.07 & 0.25 $\pm$ 0.08 & 0.23  & 14.10 & 0.05 \\
    \textbf{Average} & DepthPruning & 0.13 $\pm$ 0.04 & 0.54 $\pm$ 0.04 & 0.20  & 12.21 & 0.10 \\
    \cdashline{1-7}
    \textbf{QA} & WidthPruning & 3.25 $\pm$ 0.21 & 0.99 $\pm$ 0.23 & 0.84  & 237.08 & 0.03 \\
    \textbf{Reasoning} & WidthPruning & 0.26 $\pm$ 0.03 & 0.93 $\pm$ 0.03 & 0.62  & 72.91 & 0.11 \\
    \textbf{Language} & WidthPruning & 0.82 $\pm$ 0.05 & 0.7 $\pm$ 0.06 & 0.86  & 262.08 & 0.05 \\
    \textbf{Average} & WidthPruning & 0.39 $\pm$ 0.04 & 0.83 $\pm$ 0.04 & 0.70  & 103.11 & 0.10 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Coefficients of the method-task-level pruning laws.}
    \label{tab:method_level_full}%
\end{table}%


==> tables/model_task_level.tex <==

\begin{table}[htbp]
  \centering
  \scalebox{1}{
    \begin{tabular}{llllrrr}
      \toprule
    \bf Task  & \bf Model & \bf $\alpha$ & \bf $P_0$ & \bf Adj $R^2$ & \bf F Statistic & \bf Test Error \\
    \midrule
    \bf QA& OPT-2.7B & 2.47 $\pm$ 0.24 & 1.19 $\pm$ 0.27 & 0.93  & 106.36 & 0.02 \\
    \bf Reasoning& OPT-2.7B & 0.17 $\pm$ 0.02 & 0.96 $\pm$ 0.02 & 0.89  & 65.37 & 0.04 \\
    \bf Language& OPT-2.7B & 0.65 $\pm$ 0.02 & 0.75 $\pm$ 0.02 & 0.99  & 1268.91 & 0.01 \\
    \bf Average& OPT-2.7B & 0.28 $\pm$ 0.03 & 0.85 $\pm$ 0.03 & 0.93  & 109.53 & 0.03 \\
    \cdashline{1-7}
    \bf QA& OPT-6.7B & 2.6 $\pm$ 0.33 & 1.44 $\pm$ 0.37 & 0.88  & 61.1  & 0.05 \\
    \bf Reasoning& OPT-6.7B & 0.21 $\pm$ 0.04 & 0.96 $\pm$ 0.04 & 0.82  & 36.48 & 0.11 \\
    \bf Language& OPT-6.7B & 0.74 $\pm$ 0.09 & 0.8 $\pm$ 0.1 & 0.9   & 73.67 & 0.06 \\
    \bf Average& OPT-6.7B & 0.34 $\pm$ 0.05 & 0.87 $\pm$ 0.06 & 0.83  & 39.88 & 0.1 \\
    \cdashline{1-7}
    \bf QA& LLaMA-7B & 1.84 $\pm$ 0.12 & 1.24 $\pm$ 0.13 & 0.97  & 243.24 & 0.1 \\
    \bf Reasoning& LLaMA-7B & 0.25 $\pm$ 0.04 & 0.93 $\pm$ 0.04 & 0.85  & 47.06 & 0.08 \\
    \bf Language& LLaMA-7B & 0.71 $\pm$ 0.04 & 0.72 $\pm$ 0.04 & 0.98  & 383.52 & 0.03 \\
    \bf Average& LLaMA-7B & 0.38 $\pm$ 0.04 & 0.86 $\pm$ 0.05 & 0.9   & 74.55 & 0.07 \\
    \cdashline{1-7}
    \bf QA& OPT-13B & 2.62 $\pm$ 0.33 & 1.76 $\pm$ 0.37 & 0.88  & 61.79 & 0.06 \\
    \bf Reasoning& OPT-13B & 0.21 $\pm$ 0.01 & 0.94 $\pm$ 0.02 & 0.96  & 212.27 & 0.02 \\
    \bf Language& OPT-13B & 0.75 $\pm$ 0.03 & 0.8 $\pm$ 0.03 & 0.99  & 696.71 & 0.02 \\
    \bf Average& OPT-13B & 0.34 $\pm$ 0.02 & 0.87 $\pm$ 0.02 & 0.98  & 375.15 & 0.02 \\
    \cdashline{1-7}
    \bf QA& LLaMA-13B & 2.57 $\pm$ 0.31 & 1.74 $\pm$ 0.34 & 0.9   & 70.56 & 0.05 \\
    \bf Reasoning& LLaMA-13B & 0.28 $\pm$ 0.04 & 0.93 $\pm$ 0.04 & 0.88  & 61.4  & 0.07 \\
    \bf Language& LLaMA-13B & 0.78 $\pm$ 0.04 & 0.73 $\pm$ 0.04 & 0.98  & 492.22 & 0.03 \\
    \bf Average& LLaMA-13B & 0.4 $\pm$ 0.04 & 0.83 $\pm$ 0.04 & 0.94  & 126.08 & 0.05 \\
    
    \bottomrule
    \end{tabular}%
 }
\caption{Coefficients of the model-task-level pruning laws.}
\label{tab:model_level_full}%
\end{table}%


==> tables/number_experiments.tex <==
\begin{table*}[!htb]
\caption{Number of experiments performed in the study.}
  \centering
  \scalebox{0.85}{
    \begin{tabular}{c c c c c p{10em}}
    \cline{1-6}
    \textbf{\# Models} &\textbf{\# Methods} &  \textbf{\# Tasks} & \textbf{\# Pruning Ratios} & \textbf{\# RFT Datasize} & \textbf{\# Experiments} \\
    \cline{1-6}
    5 & 4 & 8 & 9 + 1(Base model) & 2 + 1 (No RFT) & 5 $\times$ 8 (Base) + 5 $\times$ 4 $\times$ 8 $\times$ 9 (no RFT) + 5 $\times$ 4 $\times$ 8 $\times$ 9 $\times$ 2 = 4,360\\
    \cline{1-6}
    \end{tabular}%
    }
  \label{tab:number_experiments}%
\end{table*}%


==> tables/pruned_model_results.tex <==
% Table generated by Excel2LaTeX from sheet 'pruned_results'
\begin{table}[htbp]
  \centering
  \scalebox{0.8}{
    \begin{tabular}{cccccc}
    \toprule
    \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Pruning Ratio}} & \textbf{QA} & \textbf{Reasoning} & \textbf{Language} & \textbf{Average} \\
    \toprule
    \multirow{9}[0]{*}{LLaMA-13B} & 0.1   & 0.51 $\pm$ 0.22 & 0.64 $\pm$ 0.12 & 0.46 $\pm$ 0.25 & 0.58 $\pm$ 0.16 \\
          & 0.2   & 0.41 $\pm$ 0.31 & 0.59 $\pm$ 0.14 & 0.4 $\pm$ 0.27 & 0.52 $\pm$ 0.2 \\
          & 0.3   & 0.38 $\pm$ 0.31 & 0.6 $\pm$ 0.1 & 0.39 $\pm$ 0.24 & 0.49 $\pm$ 0.19 \\
          & 0.4   & 0.34 $\pm$ 0.31 & 0.57 $\pm$ 0.12 & 0.36 $\pm$ 0.25 & 0.46 $\pm$ 0.2 \\
          & 0.5   & 0.26 $\pm$ 0.36 & 0.49 $\pm$ 0.16 & 0.3 $\pm$ 0.28 & 0.41 $\pm$ 0.22 \\
          & 0.6   & 0.21 $\pm$ 0.34 & 0.46 $\pm$ 0.14 & 0.27 $\pm$ 0.24 & 0.38 $\pm$ 0.19 \\
          & 0.7   & 0.15 $\pm$ 0.25 & 0.41 $\pm$ 0.07 & 0.18 $\pm$ 0.12 & 0.32 $\pm$ 0.1 \\
          & 0.8   & 0.01 $\pm$ 0.02 & 0.37 $\pm$ 0.01 & 0.13 $\pm$ 0.04 & 0.27 $\pm$ 0.01 \\
          & 0.9   & 0.0 $\pm$ 0.0 & 0.37 $\pm$ 0.01 & 0.09 $\pm$ 0.01 & 0.25 $\pm$ 0.01 \\
          \cdashline{1-6}
    \multirow{9}[0]{*}{LLaMA-7B} & 0.1   & 0.49 $\pm$ 0.15 & 0.61 $\pm$ 0.08 & 0.43 $\pm$ 0.22 & 0.55 $\pm$ 0.13 \\
          & 0.2   & 0.49 $\pm$ 0.14 & 0.6 $\pm$ 0.08 & 0.41 $\pm$ 0.2 & 0.54 $\pm$ 0.12 \\
          & 0.3   & 0.48 $\pm$ 0.16 & 0.59 $\pm$ 0.09 & 0.38 $\pm$ 0.19 & 0.52 $\pm$ 0.12 \\
          & 0.4   & 0.29 $\pm$ 0.31 & 0.51 $\pm$ 0.14 & 0.31 $\pm$ 0.24 & 0.43 $\pm$ 0.19 \\
          & 0.5   & 0.24 $\pm$ 0.32 & 0.48 $\pm$ 0.14 & 0.29 $\pm$ 0.23 & 0.41 $\pm$ 0.19 \\
          & 0.6   & 0.21 $\pm$ 0.33 & 0.46 $\pm$ 0.12 & 0.25 $\pm$ 0.18 & 0.37 $\pm$ 0.16 \\
          & 0.7   & 0.11 $\pm$ 0.15 & 0.4 $\pm$ 0.04 & 0.18 $\pm$ 0.08 & 0.31 $\pm$ 0.06 \\
          & 0.8   & 0.03 $\pm$ 0.03 & 0.38 $\pm$ 0.03 & 0.13 $\pm$ 0.03 & 0.27 $\pm$ 0.02 \\
          & 0.9   & 0.01 $\pm$ 0.02 & 0.38 $\pm$ 0.03 & 0.1 $\pm$ 0.03 & 0.26 $\pm$ 0.03 \\
          \cdashline{1-6}
    \multirow{9}[0]{*}{OPT-13B} & 0.1   & 0.37 $\pm$ 0.32 & 0.54 $\pm$ 0.14 & 0.39 $\pm$ 0.26 & 0.48 $\pm$ 0.19 \\
          & 0.2   & 0.35 $\pm$ 0.3 & 0.53 $\pm$ 0.14 & 0.36 $\pm$ 0.25 & 0.46 $\pm$ 0.19 \\
          & 0.3   & 0.32 $\pm$ 0.28 & 0.51 $\pm$ 0.14 & 0.33 $\pm$ 0.24 & 0.44 $\pm$ 0.18 \\
          & 0.4   & 0.28 $\pm$ 0.27 & 0.5 $\pm$ 0.13 & 0.31 $\pm$ 0.23 & 0.42 $\pm$ 0.17 \\
          & 0.5   & 0.22 $\pm$ 0.25 & 0.47 $\pm$ 0.12 & 0.28 $\pm$ 0.22 & 0.39 $\pm$ 0.16 \\
          & 0.6   & 0.17 $\pm$ 0.26 & 0.45 $\pm$ 0.11 & 0.24 $\pm$ 0.21 & 0.36 $\pm$ 0.15 \\
          & 0.7   & 0.13 $\pm$ 0.21 & 0.41 $\pm$ 0.08 & 0.2 $\pm$ 0.15 & 0.32 $\pm$ 0.11 \\
          & 0.8   & 0.01 $\pm$ 0.02 & 0.37 $\pm$ 0.03 & 0.13 $\pm$ 0.07 & 0.27 $\pm$ 0.04 \\
          & 0.9   & 0.0 $\pm$ 0.0 & 0.36 $\pm$ 0.0 & 0.07 $\pm$ 0.01 & 0.24 $\pm$ 0.0 \\
          \cdashline{1-6}
    \multirow{9}[0]{*}{OPT-2.7B} & 0.1   & 0.31 $\pm$ 0.26 & 0.51 $\pm$ 0.08 & 0.34 $\pm$ 0.19 & 0.44 $\pm$ 0.13 \\
          & 0.2   & 0.27 $\pm$ 0.23 & 0.5 $\pm$ 0.07 & 0.32 $\pm$ 0.17 & 0.43 $\pm$ 0.11 \\
          & 0.3   & 0.2 $\pm$ 0.25 & 0.49 $\pm$ 0.06 & 0.3 $\pm$ 0.16 & 0.41 $\pm$ 0.11 \\
          & 0.4   & 0.16 $\pm$ 0.25 & 0.46 $\pm$ 0.08 & 0.27 $\pm$ 0.17 & 0.37 $\pm$ 0.13 \\
          & 0.5   & 0.14 $\pm$ 0.23 & 0.43 $\pm$ 0.09 & 0.24 $\pm$ 0.18 & 0.35 $\pm$ 0.13 \\
          & 0.6   & 0.12 $\pm$ 0.19 & 0.42 $\pm$ 0.08 & 0.21 $\pm$ 0.15 & 0.33 $\pm$ 0.11 \\
          & 0.7   & 0.05 $\pm$ 0.09 & 0.39 $\pm$ 0.05 & 0.16 $\pm$ 0.1 & 0.29 $\pm$ 0.07 \\
          & 0.8   & 0.02 $\pm$ 0.03 & 0.37 $\pm$ 0.01 & 0.12 $\pm$ 0.05 & 0.26 $\pm$ 0.02 \\
          & 0.9   & 0.0 $\pm$ 0.0 & 0.36 $\pm$ 0.01 & 0.09 $\pm$ 0.01 & 0.25 $\pm$ 0.01 \\
          \cdashline{1-6}
    \multirow{9}[0]{*}{OPT-6.7B} & 0.1   & 0.52 $\pm$ 0.04 & 0.6 $\pm$ 0.01 & 0.49 $\pm$ 0.05 & 0.56 $\pm$ 0.02 \\
          & 0.2   & 0.35 $\pm$ 0.26 & 0.54 $\pm$ 0.08 & 0.38 $\pm$ 0.17 & 0.48 $\pm$ 0.12 \\
          & 0.3   & 0.13 $\pm$ 0.18 & 0.45 $\pm$ 0.11 & 0.22 $\pm$ 0.17 & 0.36 $\pm$ 0.13 \\
          & 0.4   & 0.21 $\pm$ 0.27 & 0.48 $\pm$ 0.11 & 0.31 $\pm$ 0.21 & 0.41 $\pm$ 0.15 \\
          & 0.5   & 0.17 $\pm$ 0.28 & 0.46 $\pm$ 0.11 & 0.28 $\pm$ 0.22 & 0.38 $\pm$ 0.16 \\
          & 0.6   & 0.15 $\pm$ 0.25 & 0.43 $\pm$ 0.1 & 0.24 $\pm$ 0.2 & 0.35 $\pm$ 0.14 \\
          & 0.7   & 0.1 $\pm$ 0.18 & 0.4 $\pm$ 0.07 & 0.19 $\pm$ 0.14 & 0.31 $\pm$ 0.1 \\
          & 0.8   & 0.01 $\pm$ 0.02 & 0.37 $\pm$ 0.02 & 0.12 $\pm$ 0.06 & 0.26 $\pm$ 0.03 \\
          & 0.9   & 0.0 $\pm$ 0.0 & 0.36 $\pm$ 0.0 & 0.08 $\pm$ 0.01 & 0.24 $\pm$ 0.0 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Average performance of different pruned LLMs for different pruning strategies.}
    \label{tab:pruned_model_results}%
\end{table}%


==> tables/task_level.tex <==
% Table generated by Excel2LaTeX from sheet 'task_level_fitting_laws'
\begin{table}[htbp]
  \centering
  \scalebox{0.8}{
    \begin{tabular}{lccrrr}
    \toprule
    \bf Task  & $\alpha$ & $P\_0$ & \bf Adj $R^2$ & \bf F Statistic & \bf Test Error \\
    \midrule
    QA    & 2.42 $\pm$ 0.13 & 1.45 $\pm$ 0.14 & 0.89  & 348.48 & 0.04 \\
    Reasoning & 0.22 $\pm$ 0.02 & 0.95 $\pm$ 0.02 & 0.79  & 170.83 & 0.06 \\
    Language & 0.73 $\pm$ 0.02 & 0.76 $\pm$ 0.03 & 0.96  & 947.9 & 0.03 \\
    \cdashline{1-6}
    Average & 0.35 $\pm$ 0.02 & 0.85 $\pm$ 0.02 & 0.88  & 316.37 & 0.05 \\
    \bottomrule
    \end{tabular}%
 }
  \label{tab:task_level}%
\caption{Coefficients of the task-level pruning law of the form $\mathcal{L} = \mathcal{L}_{0}P_{0}(1-r)^{\alpha}$. We report the coefficients estimated with ordinary least square (OLS) fits, along with the standard errors. To evaluate the goodness-of-fit, we calculate adjusted $R^2$, F statistic score. We calculate the test error as the average root mean square error on the test data.}
\end{table}%

